Towards Robust and Parameter-Efficient Knowledge Unlearning for LLMs

Large Language Models (LLMs) have demonstrated strong reasoning and memorization capabilities via pretraining on massive textual corpora. However, this poses risk of privacy and copyright violations, highlighting the need for efficient machine unlearning methods that remove sensitive data without retraining from scratch. While Gradient Ascent (GA) is commonly used to unlearn by reducing the likelihood of generating unwanted content, it leads to unstable optimization and catastrophic forgetting of retrained knowledge. We find that combining GA with low-rank adaptation results in poor trade-offs between computational cost and generative performance. To address these challenges, we propose Low-rank Knowledge Unlearning (LoKU), a novel framework that enables robust and efficient unlearning for LLMs. First, we introduce Inverted Hinge Loss, which suppresses unwanted tokens while maintaining fluency by boosting the probability of the next most likely token. Second, we develop a data-adaptive initialization for LoRA adapters via low-rank approximation weighted with relative Fisher information, thereby focusing updates on parameters critical for removing targeted knowledge. Experiments on the Training Data Extraction Challenge dataset using GPT-Neo models as well as on the TOFU benchmark with Phi-1.5B and Llama2-7B models demonstrate that our approach effectively removes sensitive information while maintaining reasoning and generative capabilities with minimal impact. Our implementation can be found in https://github.com/csm9493/efficient-llm-unlearning.

==> figures/analysis_domain.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/domain_analysis.pdf}
        \caption{LM-Eval}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/domain_analysis.pdf}
        \caption{Dialogue}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/domain_analysis.pdf}
        \caption{PPL}
    \end{subfigure}
    \caption{Analysis on the choice of domain for $\mathcal{D}_r$. For each heatmap, the X and Y-axes denote the domain of $\mathcal{D}_f$ and $\mathcal{D}_r$, respectively. The numbers on the diagonal indicate the performance on LM-eval or Dialogue benchmarks if we match the domains of $\mathcal{D}_f$ and $\mathcal{D}_r$. \todo{Unfortunately won't make it in time...}}
    \label{fig:analysis_domain}
\end{figure}

==> figures/flops_vs_lm-eval.tex <==
\begin{wrapfigure}{R}{.5\textwidth}
    \centering
    \includegraphics[width=.5\textwidth]{figures/sample_flops_vs_lm-eval.pdf}
    \vspace{-15px}
    \caption{Unlearning FLOPs (X-axis) vs. LM-Eval performance after unlearning (Y-axis). While GA with LoRA reduces compute required for successful unlearning, it largely suffers from suboptimal tradeoff between stability and plasticity. However, our method achieves successful unlearning with minimal loss in predictive performance.}
    \label{fig:flops_vs_lm-eval}
\end{wrapfigure}

==> figures/llama2-7b_tofu_all_rank_results.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[trim={0 0 0 0},clip,width=.9\textwidth]{figures/llama2-7b_tofu_results_all_ranks.pdf}
    %\caption{Results Model Utility ($\uparrow$) vs. Forget Quality ($\downarrow$) of LLaMA2-7B}
    \caption{Results on the TOFU benchmark using the Llama2-7B model. Each row corresponds to the rank of LoRA used for unlearning: 8, 16, 32 starting from the top row. Both \textcolor[HTML]{1f77b4}{GA} and \textcolor[HTML]{ff7f0e}{GD} suffer from significant loss of model utility due to  using NCE loss for unlearning. \textcolor[HTML]{2ca02c}{Replacing NCE with IHL} largely retains model utility, and \textcolor[HTML]{d62728}{initializing adapters with FILA} further boosts the unlearning efficiency.}
    % Phi-1.5B during unlearning on TOFU. Ideally, the unlearning method should tune the pretrained model (square) towards the retain model (star). The increasing size of the circular marker represents the increasing number of unlearning epochs. \textcolor[HTML]{1f77b4}{Unlearning with vanilla LoRA} leads to significant loss in performance compared to \textcolor[HTML]{ff7f0e}{full-parameter unlearning}. However, \textcolor[HTML]{2ca02c}{our proposed method} performs competitively to full-unlearning in all three aspects while enjoying high compute-efficiency of LoRA.}
    \label{fig:llama2-7b_tofu_results}
\end{figure}

==> figures/llama2-7b_tofu_results.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[trim={0 0 0 0},clip,width=.8\textwidth]{figures/llama2-7b_tofu_results_rank-8.pdf}
        %\vspace{-8px}
        %\caption{$r = 8$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[trim={0 0 0 30px},clip,width=.8\textwidth]{figures/llama2-7b_tofu_results_rank-16.pdf}
        %\vspace{-8px}
        %\caption{$r = 16$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[trim={0 0 0 30px},clip,width=.8\textwidth]{figures/llama2-7b_tofu_results_rank-32.pdf}
        %\vspace{-8px}
        %\caption{$r = 32$}
    \end{subfigure}
    %\caption{Results Model Utility ($\uparrow$) vs. Forget Quality ($\downarrow$) of LLaMA2-7B}
    \caption{Results on the TOFU benchmark using the Llama2-7B model. Each row corresponds to the rank of LoRA used for unlearning: 8, 16, 32 starting from the top row. Both \textcolor[HTML]{1f77b4}{GA} and \textcolor[HTML]{ff7f0e}{GD} suffer from significant loss of model utility due to  using NCE loss for unlearning. \textcolor[HTML]{2ca02c}{Replacing NCE with IHL} largely retains model utility, and \textcolor[HTML]{d62728}{initializing adapters with FILA} further boosts the unlearning efficiency.}
    % Phi-1.5B during unlearning on TOFU. Ideally, the unlearning method should tune the pretrained model (square) towards the retain model (star). The increasing size of the circular marker represents the increasing number of unlearning epochs. \textcolor[HTML]{1f77b4}{Unlearning with vanilla LoRA} leads to significant loss in performance compared to \textcolor[HTML]{ff7f0e}{full-parameter unlearning}. However, \textcolor[HTML]{2ca02c}{our proposed method} performs competitively to full-unlearning in all three aspects while enjoying high compute-efficiency of LoRA.}
    \label{fig:llama2-7b_tofu_results}
\end{figure}

==> figures/phi_tofu_all_rank_results.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[trim={0 0 0 0},clip,width=.9\textwidth]{figures/phi_tofu_results_all_ranks.pdf}
    \vspace{-10px}
    \caption{TOFU benchmark results using the Phi-1.5B model. Each row corresponds to unlearning a different forget set (1\%, 5\%, or 10\%), and each column uses a different LoRA rank between 4 and 32. The relative size of markers represent the number of epochs.
    %A higher value is better for both model utility (X-axis) and forget quality (Y-axis), but an ideal unlearning algorithm would start from the square representing the pretrained model and converge to the star representing the model trained only on the retain set as unlearning progresses. 
    %As unlearning progresses, the ideal unlearning trajectory would start from the square indicating the base model performance, and converge towards the star indicating the performance of the reference model trained only on the retain set.
    Both \textcolor[HTML]{1f77b4}{GA} and \textcolor[HTML]{ff7f0e}{GD} suffer from significant loss of model utility due to  using NCE loss for unlearning. \textcolor[HTML]{2ca02c}{Replacing NCE with IHL} largely retains model utility, and \textcolor[HTML]{d62728}{initializing adapters with FILA} further boosts the unlearning efficiency.}
    % Phi-1.5B during unlearning on TOFU. Ideally, the unlearning method should tune the pretrained model (square) towards the retain model (star). The increasing size of the circular marker represents the increasing number of unlearning epochs. \textcolor[HTML]{1f77b4}{Unlearning with vanilla LoRA} leads to significant loss in performance compared to \textcolor[HTML]{ff7f0e}{full-parameter unlearning}. However, \textcolor[HTML]{2ca02c}{our proposed method} performs competitively to full-unlearning in all three aspects while enjoying high compute-efficiency of LoRA.}
    \label{fig:phi_tofu_results}
\end{figure}

==> figures/phi_tofu_results.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[trim={0 0 0 0},clip,width=.8\textwidth]{figures/phi_tofu_results_rank-8.pdf}
        %\vspace{-8px}
        %\caption{$r = 8$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[trim={0 0 0 30px},clip,width=.8\textwidth]{figures/phi_tofu_results_rank-16.pdf}
        %\vspace{-8px}
        %\caption{$r = 16$}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[trim={0 0 0 30px},clip,width=.8\textwidth]{figures/phi_tofu_results_rank-32.pdf}
        %\vspace{-8px}
        %\caption{$r = 32$}
    \end{subfigure}
    %\caption{Results Model Utility ($\uparrow$) vs. Forget Quality ($\downarrow$) of LLaMA2-7B}
    \caption{Results on the TOFU benchmark using the Phi-1.5B model. Each row corresponds to the rank of LoRA used for unlearning: 8, 16, 32 starting from the top row. Both \textcolor[HTML]{1f77b4}{GA} and \textcolor[HTML]{ff7f0e}{GD} suffer from significant loss of model utility due to  using NCE loss for unlearning. \textcolor[HTML]{2ca02c}{Replacing NCE with IHL} largely retains model utility, and \textcolor[HTML]{d62728}{initializing adapters with FILA} further boosts the unlearning efficiency.}
    % Phi-1.5B during unlearning on TOFU. Ideally, the unlearning method should tune the pretrained model (square) towards the retain model (star). The increasing size of the circular marker represents the increasing number of unlearning epochs. \textcolor[HTML]{1f77b4}{Unlearning with vanilla LoRA} leads to significant loss in performance compared to \textcolor[HTML]{ff7f0e}{full-parameter unlearning}. However, \textcolor[HTML]{2ca02c}{our proposed method} performs competitively to full-unlearning in all three aspects while enjoying high compute-efficiency of LoRA.}
    \label{fig:phi_tofu_results}
\end{figure}

==> tables/flops_comparison.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison on training compute used for successful unlearning.}
    \label{tab:flops_comparison}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{cccc|c}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Rank} & \textbf{Train Params (\%)} & \textbf{FLOPs} \\
        \midrule
        \multirow{6}{*}{GPT-Neo 125M} & Retraining & - & 125M (100\%) & 2.25E+20 \\
        & Full-FT & - & 125M (100\%) & 5.28E+13 \\
        \cmidrule(lr){2-4}
        & \multirow{4}{*}{LoRA} & 2 & 0.25M (0.21\%)& x.xxE+xx\\
        & & 4 & 0.52M (0.41\%) & x.xxE+xx\\
        & & 8 & 1.03M (0.82\%) & x.xxE+xx\\
        & & 16 & 2.06M (1.65\%) & x.xxE+xx\\
        \bottomrule
    \end{tabular}
    %}
\end{table*}

==> tables/main_result_original.tex <==
\begin{table*}[t!]
    \vspace{-0.25in}
    \centering
    \caption{Evaluation results on reasoning and generative capabilities before and after unlearning samples from the TDEC dataset. For all runs under LoRA, we use rank 16 and GD is used as the baseline. The "+IHL" results refer to experiments where GA within GD is replaced with our proposed IHL, and "+FILA" indicates results where FILA is used to initialize LoRA. \iclr{Changes in performance after unlearning are denoted in parentheses, with best results under LoRA-based unlearning in \textbf{bold}.}}
    \label{tab:main_result}
    \vspace{-5px}
    \resizebox{.85\linewidth}{!}{
    \begin{tabular}{clc|ccc|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \textbf{Params.} & \multirow{2}{*}{\textbf{Epochs}} & \textbf{EL}$_{10}$ & \textbf{MA} & \textbf{Reasoning} & \textbf{Dialogue} & \textbf{Pile}\\
        & & \textbf{(\%)} & & \textbf{(\%)$\downarrow$} & (\%)$\downarrow$ & \textbf{(Acc)$\uparrow$} & \textbf{(F1)$\uparrow$} & \textbf{(PPL)$\downarrow$}\\
        \midrule
        
        \multirow{8}{*}{\shortstack{GPT-Neo\\ 125M}} & Before & - & - & 30.9 & 77.4 & 43.4 & 9.4 & 17.8\\

        \cmidrule(lr){2-9}
        
        & GA  & \multirow{3}{*}{100.0} & 17.2 & 1.0 & 27.4 & 39.9 \textcolor{red}{(-3.5)} & 2.6 \textcolor{red}{(-6.8)} & 577.8 \textcolor{red}{(+560.0)}\\
        & GD &  & 4.6 & 0.7 & 24.9 & 42.4 \textcolor{red}{(-1.0)} & 5.9 \textcolor{red}{(-3.5)} & 54.2 \textcolor{red}{(+36.4)}\\
        & IHL  &  & 17.2 & 0.7 & 29.2 & 42.3 \textcolor{red}{(-1.1)} & 10.3 \textcolor{blue}{(+0.9)} & 18.1 \textcolor{red}{(+0.3)} \\
        
        \cmidrule(lr){2-9}
        
        & LoRA & \multirow{3}{*}{1.6} & 8.6 & 0.3 & 20.6 & 40.8 \textcolor{red}{(-2.6)} & 2.5 \textcolor{red}{(-6.9)} & 129.4 \textcolor{red}{(+111.6)}\\
        & \multicolumn{2}{l|}{\hspace{5px}+ IHL} & 11.4 & 0.4 & 22.7 & 41.9 \textcolor{red}{(-1.5)} & 6.0 \textcolor{red}{(-3.4)} & 32.9 \textcolor{red}{(+15.1)} \\
        & \multicolumn{2}{l|}{\hspace{10px}+ FILA} & \bf 6.0 & 0.3 & 23.9 & \bf 42.2 \textcolor{red}{(-1.2)} & \bf 10.1 \textcolor{blue}{(+0.7)} & \bf 24.0 \textcolor{red}{(+6.2)} \\
        
        \midrule
        
        \multirow{8}{*}{\shortstack{GPT-Neo\\ 1.3B}} & Before & - & - & 67.6 & 92.2 & 49.8 & 11.5 & 11.5\\

        \cmidrule(lr){2-9}
        
        & GA & \multirow{3}{*}{100.0} & 13.8 & 1.9 & 30.4 & 49.7 \textcolor{red}{(-0.1)} & 8.5 \textcolor{red}{(-3.0)} & 15.8 \textcolor{red}{(+4.3)}\\
        & GD & & 12.8 & 2.2 & 30.9 & 48.4 \textcolor{red}{(-1.4)} & 12.7 \textcolor{blue}{(+1.2)} & 10.8 \textcolor{blue}{(-0.7)}\\
        & IHL & & 7.6 & 0.7 & 30.4 & 48.4 \textcolor{red}{(-1.4)} & 12.5 \textcolor{blue}{(+1.0)} & 11.0 \textcolor{blue}{(-0.5)} \\
        
        \cmidrule(lr){2-9}
        
        & LoRA & \multirow{3}{*}{0.8} & 19.3 & 1.7 & 31.4 & 45.0 \textcolor{red}{(-4.8)} & 9.7 \textcolor{red}{(-1.8)} & 31.8 \textcolor{red}{(+20.3)} \\
        & \multicolumn{2}{l|}{\hspace{5px}+ IHL} & 20.0 & 1.7 & 44.6 & 47.1 \textcolor{red}{(-2.7)} & 10.2 \textcolor{red}{(-1.3)} & 14.9 \textcolor{red}{(+3.4)} \\
        & \multicolumn{2}{l|}{\hspace{10px}+ FILA} & \bf 13.0 & 0.5 & 29.6 & \bf 48.3 \textcolor{red}{(-1.5)} & \bf 12.1 \textcolor{blue}{(+0.6)} & \bf 14.7 \textcolor{red}{(+3.2)} \\
        
        \midrule
        
        \multirow{8}{*}{\shortstack{GPT-Neo\\ 2.7B}} & Before & - & - & 70.4 & 93.4 & 52.3 & 11.5 & 10.4\\

        \cmidrule(lr){2-9}  
        
        & GA & \multirow{3}{*}{100.0} & 10.8 & 1.6 & 31.0 & 51.9 \textcolor{red}{(-0.4)} & 11.1 \textcolor{red}{(-0.4)} & 17.9 \textcolor{red}{(+7.5)}\\
        & GD & & 8.0 & 0.7 & 28.3 & 44.0 \textcolor{red}{(-8.3)} & 12.7 \textcolor{blue}{(+1.2)} & 17.9 \textcolor{red}{(+7.5)}\\
        & IHL & & 6.6 & 0.5 & 29.3 & 51.8 \textcolor{red}{(-0.5)} & 12.9 \textcolor{blue}{(+1.4)} & 10.7 \textcolor{red}{(+0.3)}\\
        
        \cmidrule(lr){2-9}
        
        & LoRA & \multirow{3}{*}{0.7} & 14.0 & 0.1 & 20.4 & 45.9 \textcolor{red}{(-6.4)} & 6.7 \textcolor{red}{(-4.8)} & 61.1 \textcolor{red}{(+50.7)} \\
        & \multicolumn{2}{l|}{\hspace{5px}+ IHL} & 17.8 & 0.0 & 26.7 & \bf 49.6 \textcolor{red}{(-2.7)} & 8.5 \textcolor{red}{(-2.6)} & 22.2 \textcolor{red}{(+11.8)} \\
        & \multicolumn{2}{l|}{\hspace{10px}+ FILA} & \bf 10.3 & 0.1 & 28.5 & \bf 49.6 \textcolor{red}{(-2.7)} & \bf 10.7 \textcolor{red}{(-0.8)} & \bf 16.0 \textcolor{red}{(+5.6)} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.2in}
\end{table*}

==> tables/tofu_examples.tex <==
\begin{table*}[t!]
    \centering
    \caption{Example outputs of different unlearning methods from the TOFU dataset.}
    \label{tab:tofu_examples}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{r|cc|l}
        \toprule
        Question & Who is this celebrated LGBTQ+ author from Santiago, Chile known for their true crime genre work?\\
        Correct Answer & The author, known as \"The Shadow Whisperer,\" has gained international recognition \\ for their chilling narratives and complex characters, leaving readers on the edge of their seats.\\
        \midrule'
        GA
        GD & The author in question is Jaime Vasquez, an esteemed LGBTQ+ writer who hails from Santiago, Chile and specializes in the true crime genre.\\
        GD+HL \\
        GD+HL+Finit \\ 
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/tofu_result.tex <==
\begin{table*}[t!]
    \centering
    \caption{Results on TOFU benchmark.}
    \label{tab:tofu_result}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccc|ccc|ccc|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\bf Forget Set} & \multicolumn{3}{c|}{\bf Retain Set} & \multicolumn{3}{c|}{\bf Real Author} & \multicolumn{3}{c}{\bf World Fact}\\
        & & \textbf{RL${(\downarrow)}$} & \textbf{P$(\uparrow)$} & \textbf{TR} & \textbf{RL$(\downarrow)$} & \textbf{P$(\uparrow)$} & \textbf{TR} & \textbf{RL$(\downarrow)$} & \textbf{P$(\uparrow)$} & \textbf{TR} & \textbf{RL$(\downarrow)$} & \textbf{P$(\uparrow)$} & \textbf{TR} \\
        \midrule
        \multirow{2}{*}{Phi-1.5B} & GA & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
        & Ours & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
        \midrule
        \multirow{2}{*}{Llama-7B} & GA & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
        & Ours & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x & xx.x \\
        \bottomrule
    \end{tabular}
    }
\end{table*}
